Improving Noise Robust Audio-Visual Speech Recognition via Router-Gated Cross-Modal Feature Fusion

Robust audio-visual speech recognition (AVSR) in noisy environments remains challenging, as existing systems struggle to estimate audio reliability and dynamically adjust modality reliance. We propose router-gated cross-modal feature fusion, a novel AVSR framework that adaptively reweights audio and visual features based on token-level acoustic corruption scores. Using an audio-visual feature fusion-based router, our method down-weights unreliable audio tokens and reinforces visual cues through gated cross-attention in each decoder layer. This enables the model to pivot toward the visual modality when audio quality deteriorates. Experiments on LRS3 demonstrate that our approach achieves an 16.51-42.67% relative reduction in word error rate compared to AV-HuBERT. Ablation studies confirm that both the router and gating mechanism contribute to improved robustness under real-world acoustic noise.

==> table/param_table.tex <==
\begin{table}[]
\caption{Parameter counts of different model configurations.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccccc@{}}
\toprule[1.5pt]
                                & \begin{tabular}[c]{@{}c@{}}AV-HuBERT \\ base\end{tabular} & \begin{tabular}[c]{@{}c@{}}AV-HuBERT \\ base (router)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Whisper-Flamingo \\ small\end{tabular} & \begin{tabular}[c]{@{}c@{}}Whisper-Flamingo \\ small (router)\end{tabular} \\ \midrule
Encoder Params. & 112M           & 112M                    & 412M                   & 412M                            \\
Decoder Params. & 114M           & 114M                    & 238M                   & 238M                            \\
Router Params.  & \xmark              & 244M                    & \xmark                      & 244M                   \\ \hline        Total Params.   & 226M           & 470M                    & 651 M                  & 895M                            
\\ \toprule[1.5pt]
\end{tabular}
}
\vspace{-2em}
\label{tab:params}
\end{table}
